GEMBA-MQM: Detecting Translation Quality Error Spans with GPT-4

This paper introduces GEMBA-MQM, a GPT-based evaluation metric designed to detect translation quality errors, specifically for the quality estimation setting without the need for human reference translations. Based on the power of large language models (LLM), GEMBA-MQM employs a fixed three-shot prompting technique, querying the GPT-4 model to mark error quality spans. Compared to previous works, our method has language-agnostic prompts, thus avoiding the need for manual prompt preparation for new languages. While preliminary results indicate that GEMBA-MQM achieves state-of-the-art accuracy for system ranking, we advise caution when using it in academic works to demonstrate improvements over other methods due to its dependence on the proprietary, black-box GPT model.

==> Makefile <==
LATEX=pdflatex
MAINFILE=thesis

default: $(MAINFILE).pdf

thesis.pdf: biblio.bib curves/trivial_progress.tex curves/parent_traces.tex curves/comparison_transfer_non.tex curves/wmt19_backtranslation.tex curves/wmt19_backtranslation_bifurcation.tex curves/example_learning_curves.tex curves/parent_drop.tex curves/low_resource_overfitting.tex curves/different_directions.tex

%.tex: %.plt
	gnuplot $< > $@

render: 
	for FILE in word_embeddings information_flow codeswitching warmstart_vocabulary; do \
		inkscape -D -z --file=img/$$FILE.svg --export-pdf=img/$$FILE.pdf --export-latex && \
		cat img/$$FILE.pdf_tex | sed "s|{$$FILE.pdf|{img/$$FILE.pdf|" > img/$$FILE.pdf_tex2 && \
		mv img/$$FILE.pdf_tex2 img/$$FILE.pdf_tex; \
	done


%.pdf: %.tex
	$(LATEX) $<
	bibtex $* || ( echo "Bibtex failed" && exit 1 )
	lim=4; \
	  while [ $$lim -ge 0 ] \
	      && grep 'Rerun to get\|Citation.*undefined' $*.log >/dev/null 2>/dev/null; do \
	    $(LATEX) $< ; \
	    lim=$$(($$lim - 1)) ; \
	  done

.PHONY: ci
ci:
	# git pull push dance with possibly uncommited local modifications
	if git pull; then echo No changes to hide; else git stash; git pull; git stash apply; fi; git commit -am pisu; git push

clean:
	rm -f $(MAINFILE).log $(MAINFILE).aux $(MAINFILE).bbl $(MAINFILE).blg $(MAINFILE).toc $(MAINFILE).out


